Geo-Adaptive Deep Spatio-Temporal predictive modeling for human mobility

Deep learning approaches for spatio-temporal prediction problems such as crowd-flow prediction assumes data to be of fixed and regular shaped tensor and face challenges of handling irregular, sparse data tensor. This poses limitations in use-case scenarios such as predicting visit counts of individuals' for a given spatial area at a particular temporal resolution using raster/image format representation of the geographical region, since the movement patterns of an individual can be largely restricted and localized to a certain part of the raster. Additionally, current deep-learning approaches for solving such problem doesn't account for the geographical awareness of a region while modelling the spatio-temporal movement patterns of an individual. To address these limitations, there is a need to develop a novel strategy and modeling approach that can handle both sparse, irregular data while incorporating geo-awareness in the model. In this paper, we make use of quadtree as the data structure for representing the image and introduce a novel geo-aware enabled deep learning layer, GA-ConvLSTM that performs the convolution operation based on a novel geo-aware module based on quadtree data structure for incorporating spatial dependencies while maintaining the recurrent mechanism for accounting for temporal dependencies. We present this approach in the context of the problem of predicting spatial behaviors of an individual (e.g., frequent visits to specific locations) through deep-learning based predictive model, GADST-Predict. Experimental results on two GPS based trace data shows that the proposed method is effective in handling frequency visits over different use-cases with considerable high accuracy.

==> samples/Tables/ablation.tex <==
%========================================================================
%Ablation study
\begin{table*}[htbp]
    \centering
    \begin{adjustbox}{width=1.0\textwidth, center=\textwidth}
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    Model name & Component 1 & Component 2 & External? & Norm. Precision & Norm. Recall\\
    \hline
    \hline
    Model 1 & $\surd$ & $\surd$ & $\surd$ & 0.40 $\pm$ 0.22 & 0.24 $\pm$ 0.25 \\  %Fused7_5_ext (DONE)
    Model 2 & $\surd$ & $\surd$ & $\times$ & 0.37 $\pm$ 0.17 & 0.22 $\pm$ 0.23 \\ %Without_ext --> Fused7_5 (DONE)
    Model 3 & $\surd$ & $\times$ & $\surd$ & 0.21 $\pm$ 0.28 & -0.02 $\pm$ 0.06 \\ %First Component with ext only --> fused7_5_ext-Comp1 (DONE)
    Model 4 & $\surd$ & $\times$ & $\times$ & \textit{nan} & -0.05 $\pm$ 0.03 \\ %First component only --> fused7_5-Comp1 (DONE)
    Model 5 & $\times$ & $\surd$ & $\surd$ & 0.37 $\pm$ 0.18 & 0.24 $\pm$ 0.22 \\  %AttOnly with ext --> Fused7_5_ext-attOnly (DONE)
    Model 6 & $\times$ & $\surd$ & $\times$ & 0.31 $\pm$ 0.14 & 0.27 $\pm$ 0.23 \\ %Att Only --> Fused7_5_attOnly (DONE)
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Different variants of \textit{GA-DSTPredict} studied using Dataset 1.} %2 x 2 grid size --> 40 x 80 --> RMS optimizer
    \label{tab:variants}
\end{table*}

==> samples/Tables/ablation2.tex <==
%========================================================================
%Ablation study
\begin{table*}[htbp]
    \centering
    \begin{adjustbox}{width=1.0\textwidth, center=\textwidth}
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    Model name & Att.\ Component & External? & Norm. Precision & Norm. Recall\\
    \hline
    \hline
    %Model 1 & $\surd$ & $\surd$ & 0.40 $\pm$ 0.22 & 0.24 $\pm$ 0.25 \\  %Fused7_5_ext (DONE)
    %Model 2 & $\surd$ & $\times$ & 0.37 $\pm$ 0.17 & 0.22 $\pm$ 0.23 \\ %Without_ext --> Fused7_5 (DONE)
    %Model 3 & $\times$ & $\surd$ & 0.21 $\pm$ 0.28 & -0.02 $\pm$ 0.06 \\ %First Component with ext only --> fused7_5_ext-Comp1 (DONE)
    %Model 4 & $\times$ & $\times$ & \textit{nan} & -0.05 $\pm$ 0.03 \\ %First component only --> fused7_5-Comp1 (DONE)
    Model 1 & $\surd$ & $\surd$ & 0.37 $\pm$ 0.18 & 0.27 $\pm$ 0.22 \\  %AttOnly with ext --> Fused7_5_ext-attOnly (DONE)
    Model 2 & $\surd$ & $\times$ & 0.30 $\pm$ 0.14 & 0.24 $\pm$ 0.23 \\ %Att Only --> Fused7_5_attOnly (DONE)
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Different variants of \textit{GA-DSTPredict} studied using Dataset 1.} %2 x 2 grid size --> 40 x 80 --> RMS optimizer
    \label{tab:variants}
\end{table*}
